AC-aware Optimization Framework for Under-Frequency Load Shedding

Under-frequency load shedding (UFLS) prevents system collapse during large disturbances. Increased penetration of distributed energy resources (DERs) and reduced system inertia makes it challenging to design a static UFLS scheme, which relies on preset frequency thresholds and load shed fractions to meet design criteria across all possible operating conditions. Due to non-linearity and traceability issues, previous adaptive UFLS schemes use simplified tractable frequency models that overlook AC network effects such as voltage-dependent load/generation. This paper leverages model order reduction techniques to obtain a higher fidelity low-order model of system frequency dynamics that captures AC network effects while incorporating turbine governor action and their associated limits. The model is then used in a new AC-aware predictive optimization framework to adapt UFLS setpoints periodically based on current operating conditions while minimizing load shed. Validated on a 1,648-bus system with PSS/E simulations, the proposed method meets design criteria under various operating conditions and disturbance scenarios. Furthermore, the framework outperforms conventional static UFLS schemes and adaptive UFLS schemes based on simplified dynamic models.

==> Sections/extras.tex <==
adaptive ---> corrective or preventive (check in citations) 

@article{MILP_UFLS_Probabilistic,
	title = {Probabilistic {Under} {Frequency} {Load} {Shedding} {Considering} {RoCoF} {Relays} of {Distributed} {Generators}},
	volume = {33},
	issn = {1558-0679},
	url = {https://ieeexplore.ieee.org/document/8241866/?arnumber=8241866},
	doi = {10.1109/TPWRS.2017.2787861},
	abstract = {The activation of under frequency load shedding (UFLS) is the last automated action against the severe frequency drops in order to rebalance the system. In this paper, the setting parameters of a multistage load shedding plan are obtained and optimized using a discretized model of dynamic system frequency response. The uncertainties of system parameters including inertia time constant, load damping, and generation deficiency are taken into account. The proposed UFLS model is formulated as a mixed-integer linear programming optimization problem to minimize the expected amount of load shedding. The activation of rate-of-change-of-frequency relays as the anti-islanding protection of distributed generators is considered. The Monte Carlo simulation method is utilized for modeling the uncertainties of system parameters. The results of probabilistic UFLS are then utilized to design four different UFLS strategies. The proposed dynamic UFLS plans are simulated over the IEEE 39-bus and the large-scale practical Iranian national grid.},
	number = {4},
	urldate = {2024-11-27},
	journal = {IEEE Transactions on Power Systems},
	author = {Amraee, Turaj and Darebaghi, Mohammad Ghaderi and Soroudi, Alireza and Keane, Andrew},
	month = jul,
	year = {2018},
	note = {Conference Name: IEEE Transactions on Power Systems},
	keywords = {Damping, Frequency response, inertia time constant, load damping, Load modeling, Power system dynamics, Relays, RoCoF, Time-frequency analysis, uncertainty, Uncertainty, Under frequency load shedding},
	pages = {3587--3598},
	file = {Full Text PDF:/Users/mazenelsaadany/Zotero/storage/4YUCLQ3R/Amraee et al. - 2018 - Probabilistic Under Frequency Load Shedding Consid.pdf:application/pdf;IEEE Xplore Abstract Record:/Users/mazenelsaadany/Zotero/storage/D7V8YUDC/8241866.html:text/html},
}


@article{FeiTeng_SFR_based_constraints,
	title = {Probabilistic {Scheduling} of {UFLS} to {Secure} {Credible} {Contingencies} in {Low} {Inertia} {Systems}},
	volume = {37},
	issn = {1558-0679},
	url = {https://ieeexplore.ieee.org/document/9599468/?arnumber=9599468},
	doi = {10.1109/TPWRS.2021.3124423},
	abstract = {The reduced inertia levels in low-carbon power grids necessitate explicit constraints to limit frequency’s nadir and rate of change during scheduling. This can result in significant curtailment of renewable energy due to the minimum generation of thermal plants that are needed to provide frequency response (FR) and inertia. Additional consideration of fast FR, a dynamically reduced largest loss and under frequency load shedding (UFLS) allows frequency security to be achieved more cost effectively. This paper derives a novel constraint from the swing equation to contain the frequency nadir using all of these services. The expected cost of UFLS is found probabilistically to facilitate its comparison to the other frequency services. We demonstrate that this constraint can be accurately and conservatively approximated for moderate UFLS levels with a second order cone (SOC), resulting in highly tractable convex problems. Case studies performed on a Great Britain 2030 system demonstrate that UFLS as an option to contain single plant outages can reduce annual operational costs by up to {\textbackslash}pounds 559 m, 52\% of frequency security costs. The sensitivity of this value to wind penetration, abundance of alternative frequency services, UFLS amount and cost is explored.},
	number = {4},
	urldate = {2024-11-17},
	journal = {IEEE Transactions on Power Systems},
	author = {O’Malley, Cormac and Badesa, Luis and Teng, Fei and Strbac, Goran},
	month = jul,
	year = {2022},
	note = {Conference Name: IEEE Transactions on Power Systems},
	keywords = {Costs, Frequency measurement, frequency response, Generators, Indexes, Inertia, Mathematical models, Security, stochastic unit commitment, Time-frequency analysis, UFLS, wind energy},
	pages = {2693--2703},
	file = {Full Text PDF:/Users/mazenelsaadany/Zotero/storage/SR6S8845/O’Malley et al. - 2022 - Probabilistic Scheduling of UFLS to Secure Credibl.pdf:application/pdf;IEEE Xplore Abstract Record:/Users/mazenelsaadany/Zotero/storage/VRLHQNVE/9599468.html:text/html},
}

@article{SFR_Original,
	title = {A low-order system frequency response model},
	volume = {5},
	issn = {1558-0679},
	url = {https://ieeexplore.ieee.org/document/65898/?arnumber=65898},
	doi = {10.1109/59.65898},
	abstract = {The authors present the derivation of a simple, low-order system frequency response (SFR) model that can be used for estimating the frequency behavior of a large power system, or islanded portion thereof, in response to sudden load disturbances. The SFR model is a simplification of other models used for this purpose, but it is believed to include the essential system dynamics. The SFR model is based on neglecting nonlinearities and all but the largest time constants in the equations of the generating units of the power system, with the added assumption that the generation is dominated by reheat steam turbine generators. This means that the generating unit inertia and reheat time constants predominate over the system average frequency response. Moreover, since only two time constants predominate, the resulting system response can be computed in closed form, thereby providing a simple, but fairly accurate, method of estimating the essential characteristics of the system frequency response.{\textless}{\textgreater}},
	number = {3},
	urldate = {2024-11-12},
	journal = {IEEE Transactions on Power Systems},
	author = {Anderson, P.M. and Mirheydar, M.},
	month = aug,
	year = {1990},
	note = {Conference Name: IEEE Transactions on Power Systems},
	keywords = {Frequency response, Turbines, Power system dynamics, Power generation, Frequency estimation, Frequency synchronization, Impedance, Nonlinear dynamical systems, Nonlinear equations, Power system modeling},
	pages = {720--729},
	file = {Full Text PDF:/Users/mazenelsaadany/Zotero/storage/MC4G6CHH/Anderson and Mirheydar - 1990 - A low-order system frequency response model.pdf:application/pdf;IEEE Xplore Abstract Record:/Users/mazenelsaadany/Zotero/storage/NSZCMLCP/65898.html:text/html},
}

@article{WAMS_based_UFLS,
	title = {{WAMS}-{Based} {Underfrequency} {Load} {Shedding} {With} {Short}-{Term} {Frequency} {Prediction}},
	volume = {31},
	issn = {1937-4208},
	url = {https://ieeexplore.ieee.org/document/7337458/?arnumber=7337458},
	doi = {10.1109/TPWRD.2015.2503734},
	abstract = {The importance of the wide-area monitoring system is rapidly increasing and many transmission system operators have already made several steps toward implementing wide-area monitoring, protection, and control. Underfrequency load shedding (UFLS) is undoubtedly one of areas that can be significantly improved within such an upgrade. However, in order to pursue finding a concept for practical implementation, as little measurements as possible should be used for the purpose. In this paper, an approach for obtaining a few-seconds-in-advance frequency prediction is described. It enables making decisions about the amount of load to be shed and, at the same time, being aware that inaccuracies in the procedure are inevitable. An extensive testing of the approach was performed on the 110 kV part of the Slovenian power-system model and the predictive UFLS appears to be highly superior to traditional UFLS on evoked frequency conditions as well as the total amount of disconnected loads. Consideration of practical limitations, such as all major time delays, unveiled a limitation for using the procedure at extreme values of system-wide frequency gradients. Consequently, the proposed algorithm is to be considered a “smart” supplement to already operational traditional UFLS.},
	number = {4},
	urldate = {2024-11-22},
	journal = {IEEE Transactions on Power Delivery},
	author = {Rudez, Urban and Mihalic, Rafael},
	month = aug,
	year = {2016},
	note = {Conference Name: IEEE Transactions on Power Delivery},
	keywords = {Adaptive control, Delay effects, Estimation, frequency response, Frequency response, Monitoring, power system islanding, Relays, Time-frequency analysis, underfrequency load shedding, wide-area measurements},
	pages = {1912--1920},
	file = {Full Text PDF:/Users/mazenelsaadany/Zotero/storage/NBT8DK5B/Rudez and Mihalic - 2016 - WAMS-Based Underfrequency Load Shedding With Short.pdf:application/pdf;IEEE Xplore Abstract Record:/Users/mazenelsaadany/Zotero/storage/27JGY8BE/7337458.html:text/html},
}


@article{Poolla_Dorfler_virtual_Inertia,
	title = {Optimal {Placement} of {Virtual} {Inertia} in {Power} {Grids}},
	volume = {62},
	issn = {1558-2523},
	url = {https://ieeexplore.ieee.org/document/7924418/?arnumber=7924418},
	doi = {10.1109/TAC.2017.2703302},
	abstract = {A major transition in the operation of electric power grids is the replacement of synchronous machines by distributed generation connected via power electronic converters. The accompanying “loss of rotational inertia” and the fluctuations by renewable sources jeopardize the system stability, as testified by the ever-growing number of frequency incidents. As a remedy, numerous studies demonstrate how virtual inertia can be emulated through various devices, but few of them address the question of “where” to place this inertia. It is, however, strongly believed that the placement of virtual inertia hugely impacts system efficiency, as demonstrated by recent case studies. In this paper, we carry out a comprehensive analysis in an attempt to address the optimal inertia placement problem. We consider a linear network-reduced power system model along with an H2 performance metric accounting for the network coherency. The optimal inertia placement problem turns out to be non-convex, yet we provide a set of closed-form global optimality results for particular problem instances as well as a computational approach resulting in locally optimal solutions. Further, we also consider the robust inertia allocation problem, wherein the optimization is carried out accounting for the worst-case disturbance location. We illustrate our results with a three-region power grid case study and compare our locally optimal solution with different placement heuristics in terms of different performance metrics.},
	number = {12},
	urldate = {2024-11-17},
	journal = {IEEE Transactions on Automatic Control},
	author = {Poolla, Bala Kameshwar and Bolognani, Saverio and Dörfler, Florian},
	month = dec,
	year = {2017},
	note = {Conference Name: IEEE Transactions on Automatic Control},
	keywords = {{\textbackslash}mathscr H\_2 norm optimization, Damping, Load modeling, optimization methods, Performance analysis, Power grids, power system dynamics, power system planning, Power system stability, Resource management, robust optimization, virtual inertia},
	pages = {6209--6220},
	file = {Full Text PDF:/Users/mazenelsaadany/Zotero/storage/3B9N7Y76/Poolla et al. - 2017 - Optimal Placement of Virtual Inertia in Power Grid.pdf:application/pdf;IEEE Xplore Abstract Record:/Users/mazenelsaadany/Zotero/storage/72EIHCZW/7924418.html:text/html},
}

@misc{NERC,
	author = {},
	title = {{PRC-006-NPCC-2} – {Automatic} {Underfrequency} {Load} {Shedding}},
	howpublished = {\url{https://www.nerc.com/pa/Stand/Reliability%20Standards/PRC-006-NPCC-2.pdf}},
	year = {},
	note = {[Accessed 27-11-2024]},
}

@article{response_based_method,
	title = {A {Data}-{Driven} {Under} {Frequency} {Load} {Shedding} {Scheme} in {Power} {Systems}},
	volume = {38},
	issn = {1558-0679},
	url = {https://ieeexplore.ieee.org/document/9767658/?arnumber=9767658},
	doi = {10.1109/TPWRS.2022.3172279},
	abstract = {This paper presents a measurement-based under-frequency load shedding scheme that considers time delays, measurement uncertainties, and communication network faults. Using a moving first-degree polynomial function, an iterative approach to estimate the frequency nadir and the associated frequency nadir time is proposed. Then, a novel method to simultaneously estimate the power imbalance and the system inertia constant is developed. According to an analytical basis, a base system is selected from a set of pre-defined base systems to guarantee accurate power imbalance estimation. Finally, a mathematical index is investigated to calculate a threshold for the generation-load power imbalance beyond which loads should be shed. Further, a systematic approach for specifying the amount of load to be shed in each transmission bus of the system is proposed. The effectiveness of the proposed methodologies is examined on both simulated and actual measured data from 9 historical power system disturbances in a national power grid.},
	number = {2},
	urldate = {2024-11-17},
	journal = {IEEE Transactions on Power Systems},
	author = {Golpîra, Hêmin and Bevrani, Hassan and Román Messina, Arturo and Francois, Bruno},
	month = mar,
	year = {2023},
	note = {Conference Name: IEEE Transactions on Power Systems},
	keywords = {Cutoff frequency, Denoising, Estimation, Frequency estimation, frequency response, Frequency response, inertia constant, measurement uncertainties, Measurement uncertainty, packet loss, Phasor measurement units, time delay, Time-frequency analysis, wide-area measurements},
	pages = {1138--1150},
	file = {Full Text PDF:/Users/mazenelsaadany/Zotero/storage/HQ3CG995/Golpîra et al. - 2023 - A Data-Driven Under Frequency Load Shedding Scheme.pdf:application/pdf;IEEE Xplore Abstract Record:/Users/mazenelsaadany/Zotero/storage/TJACCEUM/9767658.html:text/html},
}


@book{sauer_power_nodate,
	title = {{POWER} {SYSTEM} {DYNAMICS} {AND} {STABILITY}},
	language = {en},
	author = {Sauer, Peter W and Pai, M A},
	file = {Sauer and Pai - POWER SYSTEM DYNAMICS AND STABILITY.pdf:/Users/mazenelsaadany/Zotero/storage/NWSXV9KM/Sauer and Pai - POWER SYSTEM DYNAMICS AND STABILITY.pdf:application/pdf},
}


\begin{table}[htbp]
\caption{Solve Times for Different Methods and System Configurations}
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Method} & \textbf{System Configuration}       & \textbf{Solve Time (s)} \\ \hline
\multirow{3}{*}{SAFR} 
                & Base Case                           & 251.71                  \\ \cline{2-3} 
                & Reduced Inertia System              & 62.29                   \\ \cline{2-3} 
                & Penetration of DER                  & 13.29                   \\ \hline
\multirow{3}{*}{SFR} 
                & Base Case                           & 0.15                    \\ \cline{2-3} 
                & Reduced Inertia System              & 0.07                    \\ \cline{2-3} 
                & Penetration of DER                  & 0.12                    \\ \hline
\end{tabular}
\label{tab:solve_times}
\end{table}



\begin{table}[htbp]
\caption{Comparison of solve times (s) between SAFR and SFR}
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Scenario}            & \textbf{SAFR} & \textbf{SFR} \\ \midrule
Base Case                    & 251.17            & 0.15             \\
Reduced Inertia System       & 64.29             & 0.07             \\
Penetration of DER           & 13.29             & 0.12             \\ \bottomrule
\end{tabular}
\label{tab:solve_times}
\end{table}



\begin{table}[htbp]
\centering
\caption{Comparison of UFLS Schemes: Base Case}
\scriptsize
\begin{tabularx}{\columnwidth}{@{}lXXXX@{}}
\toprule
\textbf{Case}     & \textbf{Frequency Nadir (Hz)} & \textbf{Settling Frequency (Hz)} & \textbf{Load Shed (\%)}  & \textbf{Solve Time (s)} \\ \midrule
SAFR          & 58.75                 & 59.79                    & 16.79 & 251.71                    \\
SFR          & -                      & -                       & 15.58   & 0.15 \\
CONV         & 58.65                 & 59.97                    & 21.92        & -             
                  \\ \bottomrule
\end{tabularx}
\label{tab:normal_case}
\end{table}


\begin{table}[htbp]
\caption{PV Smoothing Performance Metrics }
\begin{center}
\setlength\tabcolsep{5pt}
 \centering
 %\normalsize
 \label{tab2}
\begin{tabular}{lccccc}
\toprule
{\textbf{Model}} 
 & \textbf{Solver}& \textbf{Predicted}& \textbf{Actual} &\textbf{Predicted}& \textbf{Actual} \\

 {}& \textbf{Time}& \textbf{R99}& \textbf{R99} &\textbf{MSE}& \textbf{ MSE} \\
  {}& \textbf{(s)}& \textbf{(kW/min)}& \textbf{(kW/min)} &\textbf{(kW$^2$)}& \textbf{(kW$^2$)} \\
 \toprule
NLP & 6.934 & 4.59 & 4.59 & 18.42 & 18.42 \\ 
 % \hline
 NLP WS & 5.480 & 6.33 & 6.33 & 27.30 & 27.30\\ 
  % \hline
 MIP & 0.798 & 1.10 & 1.0 & 4.69 & 4.69\\ 
 % \hline
 Relaxed & 0.025 & 1.10 & 1.15 & 4.46 & 4.79 \\ 
 % \hline
Robust & 0.028 & 1.10 & 1.10 & 5.20 & 5.20\\ 
  % \hline
Two-Stage LP & 0.037 & 1.10 & 1.10 & 4.72 & 4.72 \\ 
  \bottomrule
\end{tabular}
\end{center}
\end{table}


% , and $P_\text{UFLS}^{+}[k]$ and $P_\text{UFLS}^{-}[k]$ are the upper and lower bounds on the total UFLS load shed input to the system at timestep $k$ and are constrained as follows:
% \begin{subequations}
% \begin{align}
%     P_\text{UFLS}^{+}[k+d] &= \sum_{i=1}^{N_\text{UFLS}} P_{i}^+[k]  \label{eqn:P UFLS Power Upper} \\
%     P_\text{UFLS}^{-}[k+d] &= \sum_{i=1}^{N_\text{UFLS}} P_{i}^-[k]  ,\label{eqn:P UFLS Power Lower}
%  \end{align}
% \end{subequations}

% \begin{subequations}
% \begin{align}
%     P_\text{UFLS}^{+}[k+d] &= \sum_{i=1}^{N_\text{UFLS}} P_{i}^+[k]  \label{eqn:P UFLS Power Upper} \quad \land \quad
%     Q_\text{UFLS}^{+}[k+d] = \sum_{i=1}^{N_\text{UFLS}} Q_{i}^+[k] \\
%     P_\text{UFLS}^{-}[k+d] &= \sum_{i=1}^{N_\text{UFLS}} P_{i}^-[k]  \label{eqn:P UFLS Power Lower} \quad \land \quad
%     Q_\text{UFLS}^{-}[k+d] = \sum_{i=1}^{N_\text{UFLS}} Q_{i}^-[k],
%  \end{align}
% \end{subequations}
